The difference between molecules and materials: Reassessing the role of exact conditions in density functional theory

Exact conditions have long been used to guide the construction of density functional approximations. But hundreds of empirical-based approximations tailored for chemistry are in use, many of which neglect these conditions in their design. We analyze well-known conditions and revive several obscure ones. Two crucial distinctions are drawn: that between necessary and sufficient conditions, and between all electronic densities and the subset of realistic Coulombic ground states. Simple search algorithms find that many empirical approximations satisfy many exact conditions for realistic densities and non-empirical approximations satisfy even more conditions than those enforced in their construction. The role of exact conditions in developing approximations is revisited.

==> Burke_template.tex <==
\renewcommand{\thesection}{\arabic{section}}


\hyphenpenalty=10000
\usepackage{amsmath}
\usepackage{physics}
\usepackage{amssymb}
\usepackage{hyperref}
\usepackage{float}
\usepackage[dvipsnames]{xcolor}

\usepackage[caption=false]{subfig}
\usepackage{tabularx}
%\usepackage[justification=justified,singlelinecheck=false]{caption}
%\usepackage{subcaption}

\usepackage{graphicx}

\definecolor{TITLECOL}{rgb}{0.05,0.25,0.85}
\definecolor{CONTENTSCOL}{rgb}{0.1,0.2,0.7}
\definecolor{URLCOL}{rgb}{0,0.52,0.83}
\definecolor{LINKCOL}{rgb}{0.05,0.5,0}
\definecolor{CITECOL}{rgb}{0.25,0,0.48}
\definecolor{SECOL}{rgb}{0.07,0.31,0.80}
\definecolor{SSECOL}{rgb}{0.26,0.19,0.75}

\newcommand{\coloredtitle}[1]{\title{\textcolor{TITLECOL}{#1}}}
%\coloredtitle#1{\title{\textcolor{TITLECOL}{#1}}}
\newcommand{\coloredauthor}[1]{\author{\textcolor{CITECOL}{#1}}} 
%\renewcommand{\author}[1]{\author{\textcolor{CITECOL}{#1}}} 

%\def\tocname{\textcolor{CONTENTSCOL}{Contents}}
\renewcommand{\sec}[1]{\section{\textcolor{SECOL}{#1}}}
\newcommand{\ssec}[1]{\subsection{\textcolor{SSECOL}{#1}}}
\newcommand{\sssec}[1]{\subsubsection{\textcolor{SSSECOL}{#1}}}


\def\PublicationsLink{http://dft.uci.edu/publications.php}
\def\preprintlink{ \href{\preprintlinklocation}{\TitleOfPaper} }
\def\preprinttext{~}

%Set up header
\usepackage{fancyhdr}
\pagestyle{fancy}
\makeatletter
%header for title page
\fancypagestyle{titlepage}
{	\lhead{\textsc{\preprinttext\ ~ \href{\PublicationsLink}{~}}}
	\chead{}
	\rhead{\preprintlink}
	\lfoot{}}
%header for remainder
\chead{ \@title}
\rhead{ \preprintlink }
\lfoot{\textsc{\preprinttext\ ~ \href{\PublicationsLink}{~}}}
\makeatother
\def\preprintlink{ 
	\href{\preprintlinklocation}
        {%v\versionnumber\ - 
~}%INSERT the reference of your paper
	}
